Exploring Business Process Deviance with Sequential and Declarative Patterns

Business process deviance refers to the phenomenon whereby a subset of the executions of a business process deviate, in a negative or positive way, with respect to {their} expected or desirable outcomes. Deviant executions of a business process include those that violate compliance rules, or executions that undershoot or exceed performance targets. Deviance mining is concerned with uncovering the reasons for deviant executions by analyzing event logs stored by the systems supporting the execution of a business process. In this paper, the problem of explaining deviations in business processes is first investigated by using features based on sequential and declarative patterns, and a combination of them. Then, the explanations are further improved by leveraging the data attributes of events and traces in event logs through features based on pure data attribute values and data-aware declarative rules. The explanations characterizing the deviances are then extracted by direct and indirect methods for rule induction. Using real-life logs from multiple domains, a range of feature types and different forms of decision rules are evaluated in terms of their ability to accurately discriminate between non-deviant and deviant executions of a process as well as in terms of understandability of the final outcome returned to the users.

==> addon/claudio-macros.tex <==
\RequirePackage{rotating}

\newcommand{\sidewaysheader}[1]{\begin{sideways}{#1}\end{sideways}}
\newcommand{\sidewaysheaderpar}[2]{\begin{sideways}\parbox{#1}{\centering #2}\end{sideways}}

\RequirePackage{paralist}

\newenvironment{iiilist}%
{\begin{inparaenum}[\itshape(i)\upshape]}%
{\end{inparaenum}}

\RequirePackage{colortbl}

\newcommand{\grayrow}{\rowcolor{gray!20}} %
\newcommand{\lightgrayrow}{\rowcolor{gray!10}} %
\newcommand{\graycell}{\cellcolor{gray!30}} %

==> addon/commands-for-revision.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Highlight changes in revised manuscripts
%
% To color text
\RequirePackage{xcolor}
% To create side-notes
\RequirePackage{marginnote}
% Change the following line for larger (or narrower) side spaces
\setlength{\marginparwidth}{2cm}
% Change the following line for bigger (or smaller) fonts
\renewcommand*{\marginfont}{\footnotesize}

\newenvironment{HlRev}[1][]{%
% No hyperrefs here
\begin{NoHyper}
% Change the colour to blue
%\color{OliveGreen}%
\color{black}%
% If an argument is passed, it is used as the number of the comment in a side note
\ifx\newenvironment#1\newenvironment\else\marginnote{Comment #1}\fi%
%
}{%
% Restores the normal colour
\normalcolor%
% Restores the normal hyperref behaviour
\end{NoHyper}%
}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

% To cross-reference other documents
\usepackage{xr}
%\externaldocument[rev:]{../letter-to-referees-for-submission-3}

==> addon/macros.tex <==
%% example environment
% \newtheorem{example}{Example}[section]
%% definition environment
% \newtheorem{definition}{Definition}[section]
%% definition environment
%\newtheorem{theorem}{Theorem}
%% definition environment
%\newtheorem{lemma}{Lemma}
% \newenvironment{proof}                          % Proof environment.
%   {\trivlist\item[\hskip\labelsep\bf Proof:]}%  %   Puts "Proof:" in front of
%   {\unskip\nobreak\hfill~$\Box$\endtrivlist}    %   and box symbol after text.
%
% \newtheorem{corollary}[theorem]{Corollary}

%%%%%%%%%%%%%%%%%%%%%%%%%% Special symbols

\begingroup
\catcode`\~=11
\gdef\urltilde{\lower 0.6ex\hbox{~}}
\endgroup

%%%%%%%%%%%%%%%%%%%%%%%%%% General Math

%\newcommand{\A}{\mathcal{A}} \newcommand{\B}{\mathcal{B}}
%\newcommand{\C}{\mathcal{C}} \newcommand{\D}{\mathcal{D}}
%\newcommand{\E}{\mathcal{E}} \newcommand{\F}{\mathcal{F}}
%\newcommand{\G}{\mathcal{G}} \renewcommand{\H}{\mathcal{H}}
%\newcommand{\I}{\mathcal{I}} \newcommand{\J}{\mathcal{J}}
%\newcommand{\K}{\mathcal{K}} \renewcommand{\L}{\mathcal{L}}
%\newcommand{\M}{\mathcal{M}} \newcommand{\N}{\mathcal{N}}
%\renewcommand{\O}{\mathcal{O}} \renewcommand{\P}{\mathcal{P}}
%\newcommand{\Q}{\mathcal{Q}} \newcommand{\R}{\mathcal{R}}
%\renewcommand{\S}{\mathcal{S}} \newcommand{\T}{\mathcal{T}}
%\newcommand{\U}{\mathcal{U}}
%\newcommand{\V}{\mathcal{V}}
%\newcommand{\W}{\mathcal{W}} \newcommand{\X}{\mathcal{X}}
%\newcommand{\Y}{\mathcal{Y}} \newcommand{\Z}{\mathcal{Z}}
\newcommand{\BE}{{\mathcal{B}, \mathcal{E}}}
\newcommand{\DB}{{\mathcal{DB}}}
\newcommand{\DS}{{\mathcal{DS}}}
\newcommand{\nopar}{\texttt{no par}}
\newcommand{\db}{\texttt{par.db}}
\newcommand{\search}{\texttt{par.src.sp}}
%% ul with space between text and line

\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\La}{\Leftarrow}
%\newcommand{\lra}{\leftrightarrow}
\newcommand{\Lra}{\Leftrightarrow}
\newcommand{\lora}{\longrightarrow}
\newcommand{\Lora}{\Longrightarrow}
\newcommand{\lola}{\longleftarrow}
\newcommand{\Lola}{\Longleftarrow}
\newcommand{\lolra}{\longleftrightarrow}
\newcommand{\Lolra}{\Longleftrightarrow}
\newcommand{\ua}{\uparrow}
\newcommand{\Ua}{\Uparrow}
\newcommand{\da}{\downarrow}
\newcommand{\Da}{\Downarrow}
\newcommand{\uda}{\updownarrow}
\newcommand{\Uda}{\Updownarrow}

\newcommand{\goto}[1]{\stackrel{#1}{\lora}}

%%%%%%%%%%%%%%%%%%%%%%%%%% Relations

\newcommand{\incl}{\subseteq}
\newcommand{\imp}{\rightarrow}
%%\newcommand{\deq}{\doteq}
\newcommand{\dleq}{\dot{\leq}}                   % dotted less equal

%%%%%%%%%%%%%%%%%%%%%%%%%% Spaces

\newcommand{\per}{\mbox{\bf .}}                  % period

\newcommand{\cld}{,\ldots,}                      % ,...,
\newcommand{\ld}[1]{#1 \ldots #1}                 % #1 ... #1
\newcommand{\cd}[1]{#1 \cdots #1}                 % #1 ... #1
\newcommand{\lds}[1]{\, #1 \; \ldots \; #1 \,}    % _#1_..._#1_
\newcommand{\cds}[1]{\, #1 \; \cdots \; #1 \,}    % _#1_..._#1_

\newcommand{\dd}[2]{#1_1,\ldots,#1_{#2}}             % x1,...,xn (da da)
\newcommand{\ddd}[3]{#1_{#2_1},\ldots,#1_{#2_{#3}}}  % xi1,...,xin (da da down)
\newcommand{\dddd}[3]{#1_{11}\cld #1_{1#3_{1}}\cld #1_{#21}\cld #1_{#2#3_{#2}}}
%%                                x_11,...,x_1n,...,x_m1,...,x_mn_m

\newcommand{\ldop}[3]{#1_1 \ld{#3} #1_{#2}}   % x1 #3...#3 xn
\newcommand{\cdop}[3]{#1_1 \cd{#3} #1_{#2}}   % x1 #3...#3 xn
\newcommand{\ldsop}[3]{#1_1 \lds{#3} #1_{#2}} % x1 _#3_..._#3_ xn
\newcommand{\cdsop}[3]{#1_1 \cds{#3} #1_{#2}} % x1 _#3_..._#3_ xn

%%%%%%%%%%%%%%%%%%%%%%%%%% Delimiters

\newcommand{\quotes}[1]{{\lq\lq #1\rq\rq}}
%\newcommand{\set}[1]{\{#1\}}                      % set
\newcommand{\Set}[1]{\left\{#1\right\}}
%%\newcommand{\bigset}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\bigmid}{\Big|}
\newcommand{\card}[1]{|{#1}|}                     % cardinality of a set
\newcommand{\Card}[1]{\left| #1\right|}
\newcommand{\cards}[1]{\sharp #1}
\newcommand{\sub}[1]{[#1]}
\newcommand{\tup}[1]{\langle #1\rangle}            % tuple
\newcommand{\Tup}[1]{\left\langle #1\right\rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%% Constraints

%%\newcommand{\relc}[3]{#1#2#3}
\newcommand{\inc}[2]{#1\colon #2}

%%%%%%%%%%%%%%%%%%%%%%%%%% DL specific commands

%%%%%%%%%%%%%%%%%%%%%%%%%% Interpretation

\newcommand{\inter}[1][\I]{(\dom[#1],\Int[#1]{\cdot})}   % (dom^I,.^I)

%\newcommand{\dom}[1][\I]{\Delta^{#1}}  % delta^I (domain of interpretation \I)
\newcommand{\Int}[2][\I]{#2^{#1}}      % #2^I    (interpretation function)
\newcommand{\INT}[2][\I]{(#2)^{#1}}    % (#2)^I  (interpretation function)

%%%%%%%%%%%%%%%%%%%%%%%%%% Basic Concept forming operators

%\newcommand{\AND}{\sqcap}
%\newcommand{\OR}{\sqcup}
% \newcommand{\NOT}{\neg}
\newcommand{\ALL}[2]{\forall #1 \per #2}
 \newcommand{\SOME}[2]{\exists #1 \per #2}
 \newcommand{\SOMET}[1]{\exists #1}
\newcommand{\ALLRC}{\ALL{R}{C}}
\newcommand{\SOMERC}{\SOME{R}{C}}
\newcommand{\SOMERT}{\SOMET{R}}
\newcommand{\ATLEAST}[2]{(\geq #1 \, #2)}
\newcommand{\ATMOST}[2]{(\leq #1 \, #2)}
\newcommand{\EXACTLY}[2]{(= #1 \, #2)}
 \newcommand{\INV}[1]{#1^{-}}

%%%%%%%%%%%%%%%%%%%%%%%%%%


%%\newcommand{\BOX}[2]{\lbrack #1\rbrack #2}
%%\newcommand{\DIAM}[2]{\langle #1\rangle #2}
\newcommand{\QATMOST}[3]{(\leq #1\; \DIAM{#2}{#3})}
%%\newcommand{\true}{tt}
%%\newcommand{\false}{ff}
\newcommand{\Ident}[1]{(#1)?}
%\renewcommand{\circ}{;}


%%\newfont{\bigmathxx}{cmsy10 scaled 1440}
%%\newcommand{\bigsqcap}{\mathop{\mathop{\mbox{\bigmathxx\symbol{117}}}}}

\newcommand{\ISA}{\sqsubseteq}
\newcommand{\EQU}{\equiv}

\newcommand{\QATLEAST}[3]{(\geq #1\, #2 \per #3)}
%%%\newcommand{\QATMOST}[3]{(\leq #1\, #2 \per #3)}
%%%\newcommand{\Ident}[1]{\mathit{id}(#1)}

\newcommand{\ALCQreg}{\mathcal{ALCQ}_\mathit{reg}}
\newcommand{\PDLgm}{\mathit{PDL}_\mathit{gm}}
\newcommand{\ALC}{\mathcal{ALC}}

\newcommand{\Nat}{{\rm I\kern-.23em N}}

\newcommand{\FaCT}{\textsc{FaCT}\xspace}
\newcommand{\Racer}{\textsc{Racer}\xspace}
\newcommand{\SHIQ}{\mathcal{SHIQ}\xspace}

\newcommand{\served}{\mathsf{served}}
\newcommand{\initiated}{\mathsf{initiated}}
\newcommand{\trans}{\mathit{trans}}
%%\newcommand{\Init}{\mathsf{Init}}

\newcommand{\ecard}{\emph{e}-card\xspace}

%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro and personal command
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\eService}{\emph{e-}Service\xspace}
\newcommand{\eServices}{\emph{e-}Services\xspace}
\newcommand{\eservice}{\emph{e-}Service\xspace}
\newcommand{\eservices}{\emph{e-}Services\xspace}
\newcommand{\eGov}{\emph{e-}Government\xspace}
\newcommand{\e}{\emph{e-}}


\newcommand{\Init}{\mathit{Init}}
%%\newcommand{\init}{_{\mathit{init}}}
\newcommand{\KB}{\mathit{KB}}
\newcommand{\VA}{\mathit{VA}}
\newcommand{\VAb}{\mathbf{VA}}

\newcommand{\exec}{\mathit{exec}}
\newcommand{\change}{\mathit{Change}}
\newcommand{\eS}{\mathit{e}\S}
\newcommand{\TeS}{\T^{\eS}}
\newcommand{\Final}{\mathit{Final}}
\newcommand{\Step}{\mathit{Step}}
\newcommand{\Poss}{\mathit{Poss}}
%\newcommand{\undef}{\mathit{undef}}
\newcommand{\fin}{\mathit{fin}}
\newcommand{\comp}{\mathit{comp}}
%%\newcommand{\true}{\mathtt{true}}
%%\newcommand{\false}{\mathtt{false}}

% \newcommand{\ttrue}{\mathit{true}}
\newcommand{\ffalse}{\mathit{false}}

\newcommand{\limp}{\rightarrow}
\newcommand{\lequiv}{\leftrightarrow}
\newcommand{\conc}{\mathord{\cdot}}
\newcommand{\eword}{\varepsilon}
\newcommand{\Diam}[2]{\langle #1 \rangle #2}
\newcommand{\Boxx}[2]{[#1]#2}

\newcommand{\myi}{\emph{(i)}\xspace}
\newcommand{\myii}{\emph{(ii)}\xspace}
\newcommand{\myiii}{\emph{(iii)}\xspace}
\newcommand{\myiv}{\emph{(iv)}\xspace}
\newcommand{\myv}{\emph{(v)}\xspace}
\newcommand{\myvi}{\emph{(vi)}\xspace}

%\newcommand{\my}[1]{\emph{(#1)}\xspace}

\newcommand{\moved}{\mathit{moved}}
\newcommand{\itext}{{\mathit{ext}}}
\newcommand{\itint}{{\mathit{int}}}

\newcommand{\ES}[1]{{#1}^\itext}
\newcommand{\IS}[1]{{#1}^\itint}
\newcommand{\EA}[1]{A^\itext_{#1}}
\newcommand{\IA}[1]{A^\itint_{#1}}
\newcommand{\CG}{CG}
\newcommand{\NCG}{NCG}
\newcommand{\MNCG}{MNCG}
\newcommand{\CHOOSE}{choose(\cdot)}
\newcommand{\NDSP}{NDSP}
\newcommand{\NDS}{NDS}
\newcommand{\MNDS}{MNDS}
\newcommand{\PLAN}{\mbox{\emph{SP}}}

%% Draft delle figure
\newcommand{\figureDraft}{
\begin{tabular}{|p{7cm}|}
\hline
\vspace{4cm}\\
\hline
\end{tabular}
}


\newcommand{\ttt}{{\mathit{tt}}}
\newcommand{\fff}{{\mathit{ff}}}
\newcommand{\uuu}{{\mathit{uu}}}
\newcommand{\transA}[3]{\{#1\}#2\{#3\}}
\newcommand{\transT}[2]{\{#1\}#2}

\newcommand{\reminder}[1]{\marginpar{\mbox{$<NEW>$}} [[{\it\small #1}]]}


\newcommand{\bsy}{\boldsymbol}
\newcommand{\certans}{\rhd}

\newcommand{\Goto}[1]{\stackrel{#1}{\Longrightarrow}}
\newcommand{\mf}{\mathfrak}
\newcommand{\msf}{\mathsf}
\newcommand{\homeq}{\stackrel{h}{=}}
\newcommand{\eqmnr}{\stackrel{mnr}{=}}
\newcommand{\sseqmnr}{\stackrel{mnr}{\subseteq}}
\newcommand{\ssmnr}{\stackrel{mnr}{\subset}}


%%%%%%%%%%%
% \newcommand\BOX[1]{\lbrack #1 \rbrack}
% \newcommand\DIAM[1]{\langle #1 \rangle}
% \newcommand{\Var}{\mbox{\em Var}}
%%%%%%%%%%% Mu-Calculus Interpretation: \mf{A}, \V

\newcommand{\Moda}[1]{#1_{\V}^\mf{A}}     % argument_{\V}^\mf{A} % Giuseppe
                                        % interp. and assign. fun.
\newcommand{\Modax}[2]{#1_{\V #2}^\mf{A}} % argument_{\V}^\mf{A} % Giuseppe
                                        % interp. and modif. assign. fun.
\newcommand{\MODA}[1]{(#1)_{\V}^\mf{A}}   % (argument)_{\V}^\mf{A} % Giuseppe
                                        % interp. and assign. fun.
\newcommand{\MODAX}[2]{(#1)_{\V #2}^\mf{A}} % (argument)_{\V.}^\mf{A} % Giuseppe
                                        % interp. and modif. assign. fun.

\newcommand{\Modat}[2]{#1_{\V}^{#2}}     % argument_{\V}^\mf{A} % Giuseppe
                                        % interp. and assign. fun.
\newcommand{\MODAT}[2]{(#1)_{\V}^{#2}}   % (argument)_{\V}^\mf{A} % Giuseppe
                                        % interp. and assign. fun.

\renewcommand{\varsigma}{\mathit{R}}
%\renewcommand{\Ra}{\mathit{Tr}}

\newcommand{\Amax}{\A_{\mathit{max}}}

% \newcommand{\ex}[1]{\mathsf{#1}}
\newcommand{\actex}[1]{\mathsf{#1}}

\newcommand{\const}[1]{\C_{#1}}

%\newcommand{\bsy}[1]{\boldsymbol{#1}}
\newcommand{\brho}{\bsy{\rho}}
\newcommand{\bpi}{\bsy{\pi}}

\newcommand{\ans}[2][]{\mathit{ans}_{#1}(#2)}
\newcommand{\rew}[1]{\mathit{rew}(#1)}
\newcommand{\DO}[1]{\mathit{do}(#1)}
\newcommand{\GOTO}[1][\mf{A}]{\mathrel{\Ra_{#1}}}

%\newcommand{\conj}{\mathit{conj}}

\newcommand{\homom}[4][\C]{#3 \mathrel{\ra^{#1}_{#2}} #4}
\newcommand{\map}[2]{#1 \rightsquigarrow #2}
\newcommand{\carule}[2]{#1 \mapsto #2}

\newcommand{\dllite}{\emph{DL-Lite}\xspace}
\newcommand{\dllitef}{\emph{DL-Lite}\ensuremath{_{\mathcal{F}}}\xspace}
\newcommand{\dlliter}{\emph{DL-Lite}\ensuremath{_{\mathcal{R}}}\xspace}
\newcommand{\dllitea}{\emph{DL-Lite}\ensuremath{_{\mathcal{A}}}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\LTLthree}{{\sc ltl}$_3$}
%\newcommand{\bs}{\boldsymbol}
\newcommand{\univproj}[1]{#1_{\downarrow \forall}}
\newcommand{\existproj}[1]{#1_{\downarrow \exists}}
\newcommand{\bsl}{\backslash}
\newcommand{\prop}{\P rop}
\newcommand{\pfunct}{\mathsf{p}}
\newcommand{\ffunct}{\mathsf{f}}
\newcommand{\rfunct}{\mathsf{r}}

\newcommand{\old}{\mathsf{old}}
\newcommand{\upsphi}{\upsilon^{\Phi}}
\newcommand{\upsnotphi}{\upsilon^{\neg \Phi}}
\newcommand{\epsphi}{\epsilon^{\Phi}}
\newcommand{\epsnotphi}{\epsilon^{\neg \Phi}}

%\newcommand{\id}{\textsc{id}\xspace}
\newcommand{\ids}{\textsc{id}s\xspace}

\newcommand{\pid}{p-\textsc{id}\xspace}
\newcommand{\pids}{p-\textsc{id}s\xspace}

\newcommand{\uid}{$\forall$-\textsc{id}\xspace}
\newcommand{\uids}{$\forall$-\textsc{id}s\xspace}

\newcommand{\eid}{$\exists$-\textsc{id}\xspace}
\newcommand{\eids}{$\exists$-\textsc{id}s\xspace}

\newcommand{\cid}{c-\textsc{id}\xspace}
\newcommand{\cids}{c-\textsc{id}s\xspace}

\newcommand{\coddid}{Codd-\textsc{id}\xspace}
\newcommand{\coddids}{Codd-\textsc{id}s\xspace}

\newcommand{\offid}{offline-\textsc{id}\xspace}
\newcommand{\offids}{offline-\textsc{id}s\xspace}


\newcommand{\prun}{p-run\xspace}

\newcommand{\urun}{$\forall$-run\xspace}

\newcommand{\erun}{$\exists$-run\xspace}

\newcommand{\crun}{c-run\xspace}
\newcommand{\cruns}{c-runs\xspace}

\newcommand{\coddrun}{Codd-run\xspace}

\newcommand{\offrun}{offline-run\xspace}

\newcommand{\Buchi}{B\"{u}chi\xspace}
\renewcommand{\=}{\! = \!}

\newcommand{\nv}{\star}

\newcommand{\coddify}{\mathsf{coddify}}
\newcommand{\rep}{\mathsf{rep}}
\newcommand{\poss}{\mathsf{poss}}

\newcommand{\cin}{\! \in \!}

%% Logics
\newcommand{\FO}{{\sc fo}\xspace}
\newcommand{\LT}{{\sc lt}$_f$\xspace}
\newcommand{\LTL}{{\sc ltl}\xspace}
\newcommand{\XES}{{\sc xes}\xspace}
\newcommand{\EC}{{\sc ec}\xspace}
\newcommand{\FOLTL}{{\sc fo-ltl}\xspace}
\newcommand{\RVLTL}{{\sc rv-ltl}\xspace}
\newcommand{\LTLf}{{\sc ltl}$_f$\xspace}
\newcommand{\LTLi}{{\sc ltl}\xspace}
\newcommand{\LDL}{{\sc ldl}\xspace}
\newcommand{\add}{\mathit{ADD}}
\newcommand{\del}{\mathit{DEL}}
\newcommand{\LDLf}{{\sc ldl}$_f$\xspace}
\newcommand{\RE}{{\sc re}$_f$\xspace}
\newcommand{\PDL}{{\sc pdl}\xspace}
\newcommand{\FOLf}{{\sc fol}$_f$\xspace}
\newcommand{\MSOf}{{\sc mso}$_f$\xspace}
\newcommand{\FOL}{{\sc fol}\xspace}
\newcommand{\MSO}{{\sc mso}\xspace}
%\newcommand{\ATA}{{\sc ata}\xspace}
\newcommand{\AFW}{{\sc afw}\xspace}
\newcommand{\NFA}{{\sc nfa}\xspace}
\newcommand{\DFA}{{\sc dfa}\xspace}
\newcommand{\CTL}{{\sc ctl}\xspace}
\newcommand{\QLTL}{{\sc qltl}\xspace}
\newcommand{\muLTL}{$\mu${\sc ltl}\xspace}
\newcommand{\declare}{{\sc Declare}}
\newcommand{\fol}{\mathit{fol}}
\newcommand{\f}{\mathit{f}}
\newcommand{\g}{\mathit{g}}
\newcommand{\re}{\mathit{re}}

%% LTL
\newcommand{\Next}{\raisebox{-0.27ex}{\LARGE$\circ$}}
\newcommand{\Wnext}{\raisebox{-0.27ex}{\LARGE$\bullet$}}
%%\newcommand{\Next}{\raisebox{0.4ex}{\tiny$\bigcirc$}}
\newcommand{\Until}{\mathop{\mathcal{U}}}
\newcommand{\Release}{\mathop{\R}}
\newcommand{\Wuntil}{\mathop{\W}}
\newcommand{\true}{\mathit{true}}
%\newcommand{\false}{\mathit{false}}
\newcommand{\temptrue}{\mathit{temp\_true}}
\newcommand{\tempfalse}{\mathit{temp\_false}}
%%\newcommand{\ttrue}{\mathtt{true}}
%%\newcommand{\ffalse}{\mathtt{false}}
\newcommand{\Last}{\mathit{Last}}
\newcommand{\Ended}{\mathit{Ended}}
\newcommand{\length}{\mathit{length}}
\newcommand{\last}{\mathit{last}}
\newcommand{\nnf}{\mathit{nnf}}
\newcommand{\CL}{\mathit{CL}}
\newcommand{\MU}[2]{\mu #1.#2}
\newcommand{\NU}[2]{\nu #1.#2}
\newcommand{\BOX}[1]{ [#1]}
\newcommand{\DIAM}[1]{\langle #1 \rangle}

\endinput
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End: 

==> addon/pkgloading.tex <==
% For language-specific hyphenations etc.
\usepackage[english]{babel}
% For nice links
\usepackage{url}
% For playing with colors in tabular environments
\usepackage{colortbl}
% For math symbols, such as \nexists
%\usepackage{amssymb}
% For more math symbols, such as \mapsfrom
%\usepackage{stmaryrd}
% For advanced graphics
%% For including figures, graphicx.sty has been loaded in
%% elsarticle.cls. If you prefer to use the old commands
%% please give \usepackage{epsfig}
% For equations, arrays of equations, defining operator names, etc.
%\usepackage{amsmath}
% For cursive math
%\usepackage{mathrsfs}
% For math symbols, such as \nexists
%\usepackage{amssymb}
%% For math environments, such as "definition"
%\usepackage{amsthm}
%\theoremstyle{definition}
%\newdefinition{definition}{Definition}[section]
%\newtheorem{theorem}{Theorem}[section]
% For enumerating the line numbers
\usepackage[left]{lineno}
% For side notes, missing figures and inline to-do's
\usepackage[textsize=scriptsize,backgroundcolor=yellow!40]{todonotes}
% For specifying kewords and acronyms
%\usepackage[nonumberlist,acronym,sanitize=none]{glossaries}
%\glsdisablehyper
% For commenting out some parts of the text
%\usepackage{comment}
% For building hyperlinks
%%\usepackage[pdftex, colorlinks=true, hyperfootnotes=true, hyperindex=true,
 %           plainpages=false, pagebackref=false, pdfpagelabels=true, pdfstartview=FitH,
  %          linkcolor=blue, citecolor=blue, urlcolor=blue,
   %         bookmarks, bookmarksopen, bookmarksdepth=3]{hyperref}
% For smart references
%\usepackage[capitalise,nameinlink]{cleveref}
% To have "Figure 3(a)" in place of "Figure 3a" and  "Table 3(a)" in place of "Table 3a"
%\captionsetup[subfigure]{subrefformat=simple,labelformat=simple}
%  \renewcommand\thesubfigure{(\alph{subfigure})}
%\captionsetup[subtable]{subrefformat=simple,labelformat=simple}
%  \renewcommand\thesubtable{(\alph{subtable})}
%\Crefname{algocf}{Algorithm}{Algorithms}
% TikZ/Pgf advanced graphics
\usepackage{tkz-base}
\usetikzlibrary{decorations.pathmorphing,trees,snakes,arrows,shapes,automata}
% To use inline and other fancy list-like environments (e.g., inparaenum)
\usepackage{paralist}
% To divide a text line into multiple columns
\usepackage{multicol}
% To create good-looking book-style tables
\usepackage{booktabs}
% To play around with list environments
\usepackage{enumitem}
% To create multirow cells in tables
\usepackage{multirow}
% To create rotated cells in tables
\usepackage{rotating}
% To create enumerated lists, whose numbering is reversed
\usepackage{etaremune}
% To make algorithmic nice-looking pseudocode
%\usepackage[ruled,linesnumbered,algo2e]{algorithm2e}
%% For creating side-notes
% \usepackage{marginnote}
% For superimposing symbols over one another within math env.
%\usepackage{mathtools}
% For strange math symbols like \Dashv
%\usepackage{mathabx}
% For LaTeX if/then statements
%\usepackage{ifthen}
% For strike-through cancellations
%\usepackage[normalem]{ulem}
%% The lineno packages adds line numbers. Start line numbering with
%% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
%% for the whole article with \linenumbers.
%\usepackage{lineno}
% For highlighted text
%\usepackage{soul}
% To add dummy text
%\usepackage{lipsum}
% To have newlines in cells, with commands such as \makecell or \thead
%\usepackage{makecell}
% For a decent formatting of numbers (and a wonderful system for numeric columns in tables, ``S'')
%\usepackage{siunitx}
%\sisetup{group-separator = {,}}
% To enable text protrusion
%\usepackage{microtype} 

==> classification.tex <==
\subsection{Classification}
In machine learning, the aim of classification is to identify, based on a training set of observations, in which category a previously unseen observation belongs to \cite{alpaydin2014introduction}. A classifier is an algorithm, which implements the classification procedure. In business process deviance mining, classification techniques are widely in use (as described in Section \ref{sec:related_work}) as they allow to classify traces as normal or deviant. In this paper they play a central role in evaluating different types of features and finding characteristics, which describe differences between deviant and normal traces.

Classification approaches are usually based on two phases: a training and an evaluation phase. The training of a classifier refers to learning a mapping between observations and their categories. A common way of training classifiers is to have your dataset split into two non-overlapping partitions: training set and test set. When performing hyperparameter optimization (e.g. choosing maximum depth of a decision tree), it is often wise to also consider a third partition, often referred to as validation set, on which the hyperparameters are selected. The classifiers are then trained on training set, optionally optimized by making use of a validation set and then the final performance evaluated on a test set. Evaluation is done to measure a classifier's performance, by calculating different comparable metrics.

In this paper the observations are traces, which are encoded as vectors of numbers (encoding described in \ref{sec:approach}). Each trace has a category label of either being deviant or normal. The event log is split into partitions of training and test set.

There are many different classifiers such as perceptrons, logistic regression models, support vector machines, artificial neural networks, decision trees and rule-based learners. In this paper decision trees and rule-based learner RIPPER (described in Section \ref{bg:ripper}) were considered, which allow for simple extraction of interpretable classification rules.


\subsubsection{Decision tree}
Decision trees are one of the more popular approaches in predicting and characterizing relationships between observations and their target values \cite{Rokach:2008:DMD:1796114}. Decision trees can be used for both classification and regression tasks, namely known as classification trees and regression trees. Regression trees targets are real values (e.g. price of a property). Classification trees target values are a classes/categories (e.g. car is a sedan or an SUV). In this work the focus is on the task of classification and therefore classification trees are used.

An example of a classification tree can be seen Figure~\ref{fig:classificationtree}, where a toy decision process of either approving or disapproving a loan based on attributes of present loan application is depicted. Internal nodes are attributes, based on which a decision at that point is made. The decision either follows left or right path depending on the conditions shown on the edges. The leaves show the result of classification, which in the sample is either a rejection or an approval of a loan. For example, if an applicant has salary over 2000 and has a credit score above 5, then the loan is approved.

Since finding an optimal decision tree is often computationally infeasible, the methods of decision tree construction are mostly heuristic \cite{Rokach:2008:DMD:1796114}. The input for classification trees is a set of observations with their respective categories.
Decision tree construction algorithms mostly work recursively in a top-down and a greedy manner \cite{Rokach:2008:DMD:1796114}. At every iteration the algorithm picks an attribute and a corresponding condition, which best split the observations according to some metric. Two more common metrics are Gini impurity (it measures how often a randomly chosen observation is incorrectly classified when considering the attribute) and Information gain (it measures the purity of resulting new nodes). On each partition, which resulted from the split, the process is repeated until some stopping criterion is fulfilled. Examples of stopping criteria are the limitation on the maximum depth of the tree or when all the considered observations have the same category \cite{Rokach:2008:DMD:1796114}.

\begin{figure}[!htb]
        \centering
                \includegraphics[width=0.7\textwidth]{figures/sampledecision}
        \caption{Example of a classification tree.}
        \label{fig:classificationtree}
\end{figure}


\textbf{Decision rule} is an IF-THEN statement, which consists of a conjunction of conditions and the target prediction. An example of a decision rule could be: \textit{IF} age is above 50 \textit{AND} sex is male \textit{THEN} person is in a risk group. A single decision rule or a set of decision rules can be used to make predictions. Getting a set of decision rules can either be done in a direct or an indirect manner. Direct is when rules are extracted directly from the data and indirect when a classifier, such as a decision tree, is first trained and then rules are extracted.

Trained classification trees can be turned into a set of decision rules in a straightforward manner \cite{Rokach:2008:DMD:1796114}. Rules can be extracted by considering all the paths from a root of a decision tree to its leaves, by conjoining the decisions made along the path from the root to leaves with desired labels. The category of a leaf is the same as the majority of training observations within the leaf. The categories of the leaves will be the predicted categories for the rules. An example rule extracted from a decision tree depicted in Figure~\ref{fig:classificationtree} is: \textit{IF} Salary (EUR) <= 2000 \textit{AND} Credit score > 8 \textit{AND} Mortgage = Yes \textit{THEN} Approve loan. As this method takes a decision tree as an input, it is an indirect method for getting decision rules.

\subsubsection{RIPPER}
\label{bg:ripper}
Repeated Incremental Pruning to Produce Error Reduction (RIPPER) is a propositional rule learner first which was proposed by Cohen, W. W. as an improvement to algorithm \textit{Incremental Reduced Error Pruning} (IREP) \cite{Cohen95fasteffective}. Contrary to first building a decision tree, RIPPER learns rules directly from the data. Generalization performance of RIPPER is very competitive with a C4.5rules algorithm \cite{Cohen95fasteffective}, which is based on a well known C4.5 decision tree building algorithm \cite{Quinlan:1993:CPM:152181}. RIPPER is able to work with both nominal and continuous data. A toy ruleset which resembles RIPPER output and covers same set of rules as decision tree in Figure~\ref{fig:classificationtree} is shown in Figure~\ref{fig:ripperout}.

\begin{figure}[!htb]
        \centering
                \includegraphics[width=0.9\textwidth]{figures/ripperout}
        \caption{Sample output of RIPPER. First two lines are rules describing positive classes (Label=1). Last line shows the default rule when none of above applies (Label=0).}
        \label{fig:ripperout}
\end{figure}


\paragraph{Sequential covering.}
RIPPER is considered to be a variant of sequential covering algorithms \cite{molnar2019}, which are general procedures to learn rules one-by-one in order to create a list of decision rules. The basic scheme of sequential covering is the following one:

\begin{itemize}[noitemsep]
\item Find a good decision rule, which covers some observations;
\item Remove observations covered by the found rule;
\item Repeat until rules cover all observations or another stopping criterion (e.g. the found rule is of too low quality) is met.
\end{itemize}

The graphical overview of such procedure is shown on Figure~\ref{fig:seqcovering}.

\begin{figure}[!htb]
        \centering
                \includegraphics[width=0.7\textwidth]{figures/seqcovering}
        \caption{Feature space is sequentially covered with one rule at a time. After each rule, observations (instances) covered by that rule are removed from further consideration. \cite{molnar2019}.}
        \label{fig:seqcovering}
\end{figure}

The procedure of RIPPER is seperated into two stages: the first stage builds the initial ruleset whileas the second stage optimizes the generated rules for better generalization capabilities. The building of the initial ruleset is further done in two parts: growing and pruning. In two-class classification scenarios, that is also worked with in the paper, one class is deemed to be positive and the other negative.


\paragraph{Building the set of rules.}
In order to grow a rule, the training set of observations is first randomly split into two sets: a growing set and a pruning set, which is done in 2-to-1 ratio, with $\frac{2}{3}$ of observations in growing set and $\frac{1}{3}$ in pruning set. Growing of a rule is done greedily, by iteratively adding conditions, that maximize first-order inductive learner's (FOIL) information gain. FOIL's information gain is calculated as $\mathit{IG} = p\cdot (\log_2\frac{p}{t} - \log_2\frac{P}{T})$, where $P$ and $p$ are counts of positive observations covered by the rule before and after the addition of a condition, $T$ and $t$ are counts of total observations covered before and after. Rule is grown until it is perfect - e.g. it no longer covers negative examples (if possible).

After each rule is grown, it is immediately pruned using a procedure called reduced error pruning (REP). Pruning is done iteratively, by deleting any final sequence of conditions from the rule. The procedure is repeated until the pruning measure $V(\mathit{rule})$ no longer increases. For pruning the following measure is used: $V(\mathit{rule}) = \frac{p-n)}{p+n}$, where $p$ and $n$ are the counts of positive and negative observations covered by the rule in the pruning set.

Both negative and positive observations covered by the pruned rule are now removed from the training set and the process of growing and pruning is repeated. The stopping condition occurs when there are no more positive observations remaining, the accuracy of the rule to be added is less than 50\% or the description length of the ruleset has grown considerably when compared to the simplest ruleset. Description length is an information theoretical heuristic, which helps in balancing between maximizing accuracy on the train set and minimizing the complexity of the ruleset \cite{QUINLAN1995464}.


\paragraph{Optimizing the set of rules.}
In the optimization part every rule, in the same order in which they are found, is checked as a candidate for optimization. For every  rule two alternatives are considered: one by replacement and second by revision. For replacement, a new rule is grown and then pruned in such a way that it minimizes the error of the entire set of rules. For revision, extra conditions are added to the rule. Out of three rules: initial, replacement and revision, the one which minimizes the description length of the entire ruleset is chosen. If after optimizing the ruleset, there are some uncovered positive observations, new rules are built using the initial way of growing and pruning rules. The same optimization process can be run several times in order to further optimize the ruleset.






==> figures/declare-tikz/atmostone.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$0..1$]{\paramx};\end{tikzpicture}

==> figures/declare-tikz/participation.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$1..\ast$]{\paramx};\end{tikzpicture}

==> fullexp.tex <==
\section{In-Depth experiments}
	\begin{figure}[!t]
	\includegraphics[width=\textwidth]{figures/Rplot02.png}
	\caption{Comparing RipperK and Decision Tree for both Average Rule Length and Accuracy.}\label{fig:dtrkgoing}
\end{figure}

\begin{table}[!pt]
	\caption{$Synth_{MR/TR}$ + Decision Tree}\label{synthtree}
	%\resizebox{\textwidth}{!}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.66 & 0.55 & 0.87 & 0.69 & 0.74 & {\color{red} 0.81}  & 0.66 & 0.55 & 0.87 & 0.55 & 0.61 & 0.82 & 0.66 & 0.55 & 0.87\\
			\texttt{mr\_tr} & {\color{red} 0.61}  & 0.56 & {\color{red} 0.75}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.76 & 0.77 & 0.82 & 0.84 & 0.81 & 0.88\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00} \\
			\texttt{proc} & {\color{red} 0.81}  & {\color{red} 0.70}  & {\color{red} 0.78}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.91 & 0.86 & 0.96 & 0.91 & 0.86 & 0.96\\
			\bottomrule
	\end{tabular}}	{\tiny\begin{tabular}{l|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & {\color{red} 0.61}  & 0.70 & 0.84 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & 0.94 & \textbf{1.00}  & 0.97 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}\\
	%\end{table} \begin{table}[!tp]
	\caption{$\mathit{Synth}_{MR/TR}$ + RipperK}\label{tab:synthRipperK}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & {\color{red} 0.58}  & 0.88 & 0.82 & 0.64 & 0.82 & 0.82 & 0.66 & 0.55 & 0.73 & 0.60 & 0.61 & {\color{red} 0.72}  & 0.66 & 0.55 & 0.73\\
			\texttt{mr\_tr} & {\color{red} 0.61}  & {\color{red} 0.78}  & {\color{red} 0.78}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.83 & 0.92 & 0.92 & 0.80 & 0.91 & 0.91\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & {\color{red} 0.76}  & 0.92 & {\color{red} 0.82}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.92 & {\color{red} 0.85}  & 0.89 & 0.92 & {\color{red} 0.85}  & 0.89\\
			\bottomrule
	\end{tabular}}
	{\tiny\begin{tabular}{l|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.78 & 0.92 & 0.91 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & 0.94 & 0.94 & 0.97 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}\\
	%\end{table} \begin{table}[!tp]
	\caption{XRay + Decision Tree}\label{tab:xrayDecision Tree}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & {\color{red} 0.49}  & {\color{red} 0.38}  & 0.56 & 0.82 & 0.80 & 0.81 & 0.78 & 0.87 & 0.81 & 0.60 & 0.73 & 0.62 & 0.67 & 0.62 & 0.67\\
			\texttt{mr\_tr} & {\color{red} 0.68}  & 0.74 & {\color{red} 0.70}  & \textbf{0.85}  & 0.84 & 0.82 & 0.81 & \textbf{0.89}  & 0.82 & 0.77 & 0.87 & 0.83 & 0.81 & {\color{red} 0.68}  & 0.75\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.74 & \textbf{1.00}  & \textbf{0.50}  & 0.69 & 0.34 & \textbf{0.50}  & 0.73 & 0.25 & 0.13 & 0.56 & 0.40 & 0.25 & 0.61\\
			\bottomrule
	\end{tabular}}
	{\tiny\begin{tabular}{l|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.70 & 0.86 & {\color{red} 0.70}  & \textbf{0.85}  & 0.79 & \textbf{0.89} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & 0.13 & \textbf{0.96}  & \textbf{1.00}  & 0.38 & 0.82\\
			\bottomrule
	\end{tabular}}\\
	%\end{table} \begin{table}[!t]
	\caption{XRay + RipperK}\label{tab:xrayRipperK}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & {\color{red} 0.48}  & {\color{red} 0.50}  & {\color{red} 0.48}  & 0.75 & 0.86 & 0.82 & 0.79 & 0.87 & 0.83 & 0.56 & 0.94 & 0.60 & 0.61 & 0.54 & 0.60\\
			\texttt{mr\_tr} & {\color{red} 0.70}  & \textbf{0.91}  & {\color{red} 0.70}  & 0.89 & 0.84 & 0.85 & \textbf{0.90}  & 0.84 & \textbf{0.88}  & 0.73 & 0.79 & 0.71 & 0.80 & {\color{red} 0.73}  & 0.77\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.84 & 0.63 & 0.82 & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.34 & 0.13 & 0.56\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.78 & \textbf{0.91}  & 0.80 & \textbf{0.90}  & 0.84 & 0.86\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & 0.50 & 0.76 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
\end{table}



\begin{table}
	\caption{Sepsis Dataset + Decision Tree}\label{tab:sepsisDecision Tree}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.87 & 0.93 & 0.96 & 0.95 & 0.93 & 0.95 & 0.84 & 0.91 & 0.90 & 0.99 & 0.99 & 0.99 & 0.86 & 0.88 & 0.97\\
			\texttt{mr\_tr} & 0.45 & {\color{red} 0.40}  & 0.74 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.94 & 0.71 & 0.97 & 0.90 & 0.86 & 0.92\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.29 & 0.23 & 0.62 & 0.34 & {\color{red} 0.12}  & 0.55 & {\color{red} 0.25}  & {\color{red} 0.12}  & {\color{red} 0.53}  & \textbf{1.00}  & 0.34 & 0.63 & 0.34 & 0.23 & 0.61\\
			\texttt{proc} & 0.64 & 0.68 & 0.77 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.91 & 0.90 & 0.93 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.68}  & {\color{red} 0.64}  & {\color{red} 0.74}  & 0.99 & 0.91 & 0.95\\
			\texttt{mr\_tr} & 0.86 & \textbf{1.00}  & 0.97 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.42}  & 0.44 & 0.67 & 0.88 & 0.86 & 0.91\\
			\texttt{mra\_tra} & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & {\color{red} 0.98}  & 0.98 & {\color{red} 0.97}  & \textbf{1.00}  & 0.99 & \textbf{1.00} \\
			\texttt{payload} & \textbf{1.00}  & {\color{red} 0.12}  & 0.72 & \textbf{1.00}  & 0.23 & 0.62 & 0.88 & 0.78 & 0.89 & \textbf{1.00}  & 0.67 & 0.84\\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.52}  & {\color{red} 0.53}  & {\color{red} 0.64}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.85 & 0.82 & 0.88 & 0.91 & 0.88 & 0.92 & 0.86 & 0.86 & 0.89 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & 0.85 & 0.88 & 0.94\\
			\texttt{mr\_tr} & 0.44 & 0.47 & {\color{red} 0.63}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.94 & 0.71 & 0.97 & 0.90 & 0.86 & 0.97\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.88 & 0.78 & 0.89 & 0.89 & \textbf{0.89}  & \textbf{0.95}  & 0.86 & 0.67 & 0.89 & 0.84 & 0.56 & 0.78 & 0.88 & 0.78 & 0.89\\
			\texttt{proc} & 0.54 & {\color{red} 0.53}  & 0.65 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.92 & 0.99 & 0.97 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.97 & 0.91 & 0.95 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.97 & 0.91 & 0.95 & 0.99 & 0.91 & 0.95\\
			\texttt{mr\_tr} & 0.86 & \textbf{1.00}  & 0.97 & 0.88 & 0.83 & 0.90 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & 0.99 & {\color{red} 0.97}  & 0.98 & \textbf{1.00}  & 0.99 & \textbf{1.00} \\
			\texttt{payload} & \textbf{1.00}  & 0.56 & 0.78 & \textbf{1.00}  & 0.67 & 0.84 & 0.86 & 0.67 & 0.83 & \textbf{1.00}  & 0.67 & 0.84 & \textbf{1.00}  & 0.67 & 0.84\\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	\caption{Sepsis Dataset + RipperK}\label{tab:sepsisRipperK}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.88 & \textbf{1.00}  & 0.97 & 0.92 & 0.93 & 0.96 & 0.86 & 0.99 & 0.96 & 0.99 & 0.99 & 0.99 & 0.82 & 0.91 & 0.91\\
			\texttt{mr\_tr} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.94 & 0.74 & 0.86 & 0.86 & 0.83 & 0.90\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00} \\
			\texttt{payload} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.48 & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50\\
			\texttt{proc} & 0.63 & 0.75 & 0.77 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.95 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & 0.99 & \textbf{1.00}  & 0.99 & 0.93 & 0.96 & {\color{red} 0.72}  & {\color{red} 0.75}  & {\color{red} 0.80}  & 0.99 & 0.91 & 0.96\\
			\texttt{mr\_tr} & 0.87 & 0.93 & 0.94 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.81 & 0.93 & 0.95\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.98 & 0.99 & {\color{red} 0.98}  & 0.97 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.90 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.67 & 0.84\\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.49}  & {\color{red} 0.40}  & {\color{red} 0.59}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.85 & 0.88 & 0.90 & \textbf{1.00}  & 0.97 & 0.99 & 0.83 & 0.77 & 0.84 & 0.99 & 0.91 & 0.95 & 0.85 & 0.90 & 0.90\\
			\texttt{mr\_tr} & 0.47 & 0.30 & 0.59 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.88 & 0.83 & 0.91 & 0.78 & 0.93 & 0.95\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.90 & \textbf{1.00}  & \textbf{1.00}  & 0.90 & \textbf{1.00}  & \textbf{1.00}  & 0.90 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.45 & 0.73 & 0.90 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & 0.55 & \textbf{1.00}  & 0.78 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.94 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.99 & 0.93 & 0.96 & \textbf{1.00}  & 0.91 & 0.96 & 0.99 & 0.93 & 0.96 & 0.98 & 0.90 & 0.95 & 0.97 & 0.93 & 0.97\\
			\texttt{mr\_tr} & 0.84 & 0.88 & 0.93 & 0.84 & \textbf{1.00}  & 0.97 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & 0.99 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.98 & 0.99 & {\color{red} 0.98}  & 0.98 & {\color{red} 0.98}  & \textbf{1.00}  & {\color{red} 0.94}  & 0.99\\
			\texttt{payload} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.67 & 0.84 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.67 & 0.84 & \textbf{1.00}  & 0.45 & 0.73\\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
\end{table}

\begin{table}
	\caption{Traffic Fine Management Process + Decision Tree}\label{tab:trafficDecision Tree}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			
			\texttt{decl} & 0.84 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.84 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.84 & 0.99 & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Art157} & {\color{red} 0.51}  & {\color{red} 0.35}  & 0.55 & {\color{red} 0.51}  & 0.37 & 0.55 & {\color{red} 0.51}  & {\color{red} 0.35}  & 0.55 & {\color{red} 0.51}  & 0.37 & 0.55 & {\color{red} 0.51}  & {\color{red} 0.35}  & 0.55\\
			\texttt{p\_Pay36} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.86}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.86}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.86}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.86}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.86} \\
			\texttt{proc} & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.82}  & 0.98 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.79}  & {\color{red} 0.79}  & {\color{red} 0.93}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Art157} & {\color{red} 0.51}  & {\color{red} 0.35}  & 0.55 & {\color{red} 0.51}  & 0.37 & 0.55 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Pay36} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.86}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.86}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			
			\texttt{decl} & 0.84 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.84 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.85 & {\color{red} 0.96}  & {\color{red} 0.98} \\
			\texttt{mr\_tr} & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Art157} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Pay36} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Art157} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Pay36} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	
	
	\caption{Traffic Fine Management Process + RipperK}\label{tab:trafficRipperK}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			
			\texttt{decl} & 0.84 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.84 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.84 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Art157} & {\color{red} 0.51}  & {\color{red} 0.35}  & {\color{red} 0.54}  & {\color{red} 0.51}  & 0.36 & {\color{red} 0.54}  & {\color{red} 0.51}  & {\color{red} 0.35}  & {\color{red} 0.54}  & {\color{red} 0.51}  & 0.37 & {\color{red} 0.54}  & {\color{red} 0.51}  & {\color{red} 0.35}  & {\color{red} 0.54} \\
			\texttt{p\_Pay36} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.50}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.50}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.50}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.50}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.50} \\
			\texttt{proc} & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.82}  & {\color{red} 0.99}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.77}  & {\color{red} 0.98}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Art157} & {\color{red} 0.51}  & 0.37 & {\color{red} 0.54}  & {\color{red} 0.51}  & 0.38 & {\color{red} 0.54}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Pay36} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.50}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.50}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			
			\texttt{decl} & 0.84 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.84 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.84 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Art157} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Pay36} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Art157} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_Pay36} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
\end{table}



\begin{table}
	\caption{BPI Challenge 2011 + Decision Tree}\label{tab:bpi11Decision Tree}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{0.90}  & \textbf{0.76}  & \textbf{0.86}  & 0.80 & \textbf{0.76}  & 0.85 & 0.81 & 0.70 & 0.83 & 0.79 & 0.73 & 0.84 & 0.82 & 0.73 & 0.84\\
			\texttt{mr\_tr} & \textbf{1.00}  & 0.99 & 0.99 & 0.97 & {\color{red} 0.95}  & {\color{red} 0.95}  & \textbf{1.00}  & 0.99 & 0.99 & 0.98 & 0.99 & 0.97 & \textbf{1.00}  & 0.99 & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_M13} & 0.57 & 0.57 & 0.84 & 0.34 & {\color{red} 0.17}  & 0.83 & 0.38 & 0.44 & 0.82 & {\color{red} 0.29}  & 0.20 & 0.81 & 0.38 & 0.37 & {\color{red} 0.70} \\
			
			\texttt{p\_T101} & 0.77 & 0.65 & 0.83 & {\color{red} 0.65}  & 0.71 & 0.81 & 0.73 & 0.68 & 0.81 & 0.72 & 0.81 & 0.87 & {\color{red} 0.65}  & 0.71 & 0.84\\
			
			\texttt{proc} & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.60 & 0.73 & 0.83 & 0.60 & 0.73 & 0.83 & 0.55 & 0.53 & {\color{red} 0.73}  & {\color{red} 0.50}  & {\color{red} 0.37}  & 0.76\\
			\texttt{mr\_tr} & 0.98 & \textbf{1.00}  & \textbf{1.00}  & 0.98 & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.95}  & 0.98 & {\color{red} 0.95}  & 0.98 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.95}  & {\color{red} 0.93}  & {\color{red} 0.94}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_M13} & 0.70 & 0.31 & \textbf{0.86}  & 0.67 & 0.27 & 0.84 & 0.73 & 0.61 & 0.79 & 0.61 & 0.57 & 0.78\\
			
			\texttt{p\_T101} & 0.67 & 0.59 & 0.84 & {\color{red} 0.65}  & {\color{red} 0.52}  & {\color{red} 0.79}  & 0.88 & 0.94 & 0.97 & 0.79 & 0.71 & 0.84\\
			
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & {\color{red} 0.93}  & {\color{red} 0.92}  & {\color{red} 0.92}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.85 & \textbf{0.76}  & \textbf{0.86}  & 0.84 & 0.73 & 0.85 & 0.76 & \textbf{0.76}  & 0.85 & 0.78 & \textbf{0.76}  & 0.85 & \textbf{0.90}  & 0.73 & 0.85\\
			\texttt{mr\_tr} & \textbf{1.00}  & 0.99 & 0.99 & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.99 & 0.99 & 0.99 & 0.98 & 0.98 & \textbf{1.00}  & 0.99 & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_M13} & 0.76 & 0.61 & 0.78 & 0.67 & 0.61 & 0.77 & 0.70 & 0.61 & 0.78 & 0.68 & \textbf{0.70}  & 0.82 & 0.66 & 0.57 & 0.76\\
			
			\texttt{p\_T101} & 0.82 & 0.88 & 0.92 & 0.80 & 0.88 & 0.92 & 0.82 & 0.88 & 0.92 & 0.83 & 0.91 & 0.93 & 0.84 & \textbf{0.97}  & \textbf{0.98} \\
			
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.60 & 0.73 & 0.83 & {\color{red} 0.50}  & 0.39 & 0.77 & 0.60 & 0.73 & 0.83 & {\color{red} 0.50}  & 0.39 & 0.78 & {\color{red} 0.50}  & {\color{red} 0.37}  & 0.76\\
			\texttt{mr\_tr} & 0.98 & \textbf{1.00}  & \textbf{1.00}  & 0.98 & \textbf{1.00}  & \textbf{1.00}  & 0.98 & \textbf{1.00}  & \textbf{1.00}  & 0.98 & \textbf{1.00}  & \textbf{1.00}  & 0.98 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_M13} & 0.59 & 0.61 & 0.76 & \textbf{0.78}  & 0.57 & 0.78 & 0.61 & 0.50 & 0.76 & 0.62 & 0.54 & 0.75 & 0.66 & 0.50 & {\color{red} 0.70} \\
			
			\texttt{p\_T101} & 0.82 & 0.84 & 0.90 & \textbf{0.89}  & 0.75 & 0.87 & 0.79 & 0.84 & 0.90 & 0.87 & 0.81 & 0.89 & 0.76 & 0.78 & 0.86\\
			
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	\caption{BPI Challenge 2011 + RipperK}\label{tab:bpi11RipperK}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.90 & 0.73 & 0.86 & 0.90 & 0.73 & 0.86 & 0.90 & 0.73 & 0.86 & 0.90 & 0.73 & 0.86 & 0.90 & 0.73 & 0.86\\
			\texttt{mr\_tr} & 0.97 & \textbf{1.00}  & 0.98 & \textbf{1.00}  & 0.99 & 0.99 & 0.98 & 0.99 & 0.98 & 0.98 & \textbf{1.00}  & 0.98 & 0.98 & \textbf{1.00}  & 0.98\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_M13} & 0.62 & {\color{red} 0.27}  & {\color{red} 0.62}  & 0.74 & 0.37 & 0.67 & 0.49 & 0.50 & 0.70 & 0.61 & 0.31 & 0.63 & {\color{red} 0.47}  & 0.47 & 0.68\\
			
			\texttt{p\_T101} & 0.68 & 0.75 & 0.85 & 0.76 & 0.71 & 0.84 & 0.72 & 0.75 & 0.85 & 0.75 & 0.75 & 0.85 & {\color{red} 0.65}  & 0.78 & 0.84\\
			
			\texttt{proc} & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.58}  & {\color{red} 0.62}  & {\color{red} 0.76}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.99 & 0.99 & 0.98 & 0.98 & \textbf{1.00}  & 0.98 & {\color{red} 0.96}  & \textbf{1.00}  & {\color{red} 0.96}  & 0.98 & 0.99 & 0.98\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.95}  & {\color{red} 0.98}  & {\color{red} 0.95}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_M13} & 0.64 & 0.47 & 0.71 & 0.58 & 0.37 & 0.66 & 0.71 & 0.57 & 0.77 & \textbf{0.85}  & 0.54 & 0.76\\
			
			\texttt{p\_T101} & 0.75 & 0.75 & 0.85 & 0.71 & 0.71 & 0.83 & 0.72 & 0.88 & 0.92 & 0.83 & 0.78 & 0.87\\
			
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.92}  & {\color{red} 0.95}  & {\color{red} 0.95}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.83 & 0.67 & 0.82 & 0.85 & 0.78 & 0.88 & 0.85 & 0.76 & 0.87 & 0.89 & 0.67 & 0.83 & 0.83 & 0.78 & 0.87\\
			\texttt{mr\_tr} & 0.99 & 0.97 & 0.98 & 0.98 & 0.99 & 0.97 & \textbf{1.00}  & 0.98 & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.96}  & 0.99 & \textbf{1.00}  & {\color{red} 0.96}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_M13} & 0.58 & 0.40 & 0.68 & 0.63 & 0.50 & 0.73 & 0.69 & 0.50 & 0.74 & 0.69 & 0.50 & 0.74 & 0.66 & 0.57 & 0.76\\
			\texttt{p\_T101} & 0.76 & 0.97 & 0.96 & 0.84 & \textbf{1.00}  & \textbf{0.98}  & 0.71 & 0.84 & 0.89 & 0.74 & 0.97 & 0.95 & \textbf{0.89}  & 0.97 & \textbf{0.98} \\
			\texttt{proc} & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.99 & 0.99 & 0.98 & 0.97 & 0.99 & 0.97 & 0.98 & \textbf{1.00}  & 0.98 & 0.98 & 0.98 & 0.98 & 0.99 & 0.97 & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_M13} & 0.74 & 0.47 & 0.72 & 0.77 & 0.54 & 0.76 & 0.59 & \textbf{0.70}  & \textbf{0.80}  & 0.67 & 0.54 & 0.75 & 0.74 & 0.64 & \textbf{0.80} \\
			
			\texttt{p\_T101} & 0.77 & {\color{red} 0.65}  & 0.81 & 0.80 & {\color{red} 0.65}  & {\color{red} 0.80}  & 0.71 & 0.71 & 0.83 & 0.78 & 0.68 & 0.83 & 0.73 & 0.78 & 0.87\\
			
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.97 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.97 & 0.99\\
			\bottomrule
	\end{tabular}}
	
	
\end{table}


\begin{table}
	\caption{BPI Challenge 2012 + Decision Tree}\label{tab:bpi12_Decision Tree}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & {\color{red} 0.61}  & 0.84 & 0.93 & 0.92 & 0.89 & \textbf{1.00}  & 0.62 & 0.66 & {\color{red} 0.84}  & 0.95 & 0.91 & \textbf{1.00}  & 0.63 & 0.89 & 0.93\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_45000} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.36}  & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.55 & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.36}  & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.53 & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.36} \\
			\texttt{p\_6500} & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.49 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.53 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.47 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.48 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.51\\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.61}  & {\color{red} 0.02}  & 0.86 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.69}  & {\color{red} 0.54}  & {\color{red} 0.94}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.67}  & 0.28 & {\color{red} 0.84}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_45000} & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.74 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.55 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_6500} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.43}  & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.48 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.66}  & {\color{red} 0.31}  & {\color{red} 0.87}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & 0.62 & \textbf{1.00}  & 0.97 & 0.95 & 0.86 & \textbf{1.00}  & 0.62 & 0.77 & 0.93 & 0.92 & 0.92 & 0.98 & 0.62 & 0.89 & 0.96\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_45000} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_6500} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_45000} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_6500} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.95 & 0.98 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	\caption{bpi12 + RipperK}\label{tab:bpi12_RipperK}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			
			\texttt{decl} & 0.63 & \textbf{1.00}  & 0.97 & 0.92 & 0.86 & 0.93 & 0.63 & \textbf{1.00}  & 0.97 & 0.96 & 0.92 & 0.96 & 0.63 & \textbf{1.00}  & 0.97\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_45000} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50\\
			\texttt{p\_6500} & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.53}  & {\color{red} 0.11}  & 0.55 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.69}  & {\color{red} 0.62}  & {\color{red} 0.79}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.68}  & {\color{red} 0.30}  & {\color{red} 0.64}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_45000} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_6500} & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.50 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.62}  & {\color{red} 0.40}  & {\color{red} 0.67}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			
			\texttt{decl} & 0.63 & \textbf{1.00}  & 0.97 & 0.97 & 0.84 & 0.92 & 0.63 & \textbf{1.00}  & 0.97 & 0.97 & 0.85 & 0.93 & 0.63 & \textbf{1.00}  & 0.97\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_45000} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_6500} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_45000} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{p\_6500} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.95 & 0.98 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}	
\end{table}


%\begin{table}
%	\caption{bpi17 + Decision Tree}\label{tab:bpi17Decision Tree}
%	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
%			\toprule
%			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
%			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
%			\midrule
%			\texttt{decl1} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{p\_A} & {\color{red} 0.77}  & 0.91 & {\color{red} 0.67}  & {\color{red} 0.77}  & 0.91 & {\color{red} 0.67}  & {\color{red} 0.77}  & 0.91 & {\color{red} 0.67}  & {\color{red} 0.77}  & 0.91 & {\color{red} 0.67}  & {\color{red} 0.77}  & 0.91 & {\color{red} 0.67} \\
%			\bottomrule
%	\end{tabular}}
%	
%	
%	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
%			\toprule
%			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
%			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
%			\midrule
%			\texttt{decl1} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.96}  & {\color{red} 0.95}  & {\color{red} 0.98}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.97}  & {\color{red} 0.97}  & {\color{red} 0.98}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.92}  & {\color{red} 0.98}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{p\_A} & {\color{red} 0.77}  & 0.91 & {\color{red} 0.67}  & {\color{red} 0.77}  & 0.91 & {\color{red} 0.67}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\bottomrule
%	\end{tabular}}
%	
%	
%	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
%			\toprule
%			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
%			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
%			\midrule
%			\texttt{decl1} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{p\_A} & 0.80 & {\color{red} 0.90}  & 0.73 & 0.78 & 0.92 & 0.75 & 0.80 & {\color{red} 0.90}  & 0.73 & 0.78 & 0.92 & 0.75 & 0.80 & {\color{red} 0.90}  & 0.73\\
%			\bottomrule
%	\end{tabular}}
%	
%	
%	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
%			\toprule
%			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
%			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
%			\midrule
%			\texttt{decl1} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{p\_A} & 0.80 & {\color{red} 0.90}  & 0.73 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.78 & 0.93 & 0.75 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\bottomrule
%	\end{tabular}}
%	
%	\caption{bpi17 + RipperK}\label{tab:bpi17RipperK}
%	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
%			\toprule
%			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
%			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
%			\midrule
%			\texttt{decl1} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{p\_A} & {\color{red} 0.77}  & {\color{red} 0.91}  & {\color{red} 0.63}  & {\color{red} 0.77}  & {\color{red} 0.91}  & {\color{red} 0.63}  & {\color{red} 0.77}  & {\color{red} 0.91}  & {\color{red} 0.63}  & {\color{red} 0.77}  & {\color{red} 0.91}  & {\color{red} 0.63}  & {\color{red} 0.77}  & {\color{red} 0.91}  & {\color{red} 0.63} \\
%			\bottomrule
%	\end{tabular}}
%	
%	
%	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
%			\toprule
%			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
%			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
%			\midrule
%			\texttt{decl1} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.96}  & {\color{red} 0.95}  & {\color{red} 0.95}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.98}  & {\color{red} 0.96}  & {\color{red} 0.98}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.91}  & {\color{red} 0.98}  & {\color{red} 0.98}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{p\_A} & {\color{red} 0.77}  & {\color{red} 0.91}  & {\color{red} 0.63}  & {\color{red} 0.77}  & {\color{red} 0.91}  & {\color{red} 0.63}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\bottomrule
%	\end{tabular}}
%	
%	
%	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
%			\toprule
%			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
%			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
%			\midrule
%			\texttt{decl1} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{p\_A} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\bottomrule
%	\end{tabular}}
%	
%	
%	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
%			\toprule
%			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
%			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
%			\midrule
%			\texttt{decl1} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\texttt{p\_A} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
%			\bottomrule
%	\end{tabular}}
%\end{table}


\begin{table}
	\caption{BPI Challenge 2015, Sub-Dataset A + Decision Tree}\label{tab:BPIc15SubADecision Tree}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & 0.97 & \textbf{1.00}  & 0.97 & 0.96 & 0.99 & 0.96 & 0.96 & \textbf{1.00}  & 0.96 & 0.96 & 0.99 & 0.96 & 0.96 & \textbf{1.00}  & 0.96\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & 0.99 & 0.99 & \textbf{1.00}  & 0.99 & 0.99 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & {\color{red} 0.19}  & {\color{red} 0.17}  & 0.55 & 0.48 & 0.20 & 0.62 & 0.23 & {\color{red} 0.17}  & 0.58 & 0.40 & {\color{red} 0.17}  & 0.59 & 0.27 & 0.20 & 0.57\\
			\texttt{proc} & 0.81 & 0.53 & 0.87 & \textbf{1.00}  & 0.98 & \textbf{0.99}  & 0.81 & 0.59 & 0.91 & \textbf{1.00}  & 0.92 & \textbf{0.99}  & 0.89 & 0.65 & 0.88\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.81}  & {\color{red} 0.82}  & {\color{red} 0.73}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.75}  & {\color{red} 0.77}  & {\color{red} 0.67}  & 0.99 & \textbf{1.00}  & 0.99\\
			\texttt{mr\_tr} & {\color{red} 0.73}  & \textbf{1.00}  & {\color{red} 0.76}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.77 & {\color{red} 0.73}  & 0.77 & 0.99 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.90}  & {\color{red} 0.96}  & {\color{red} 0.88}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.44 & \textbf{1.00}  & 0.89 & 0.44 & \textbf{1.00}  & 0.89 & \textbf{0.98}  & 0.89 & \textbf{0.95}  & 0.44 & \textbf{1.00}  & 0.89\\
			\texttt{proc} & 0.44 & \textbf{1.00}  & 0.90 & 0.44 & \textbf{1.00}  & 0.90 & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.51}  & 0.44 & \textbf{1.00}  & 0.90\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & 0.97 & 0.99 & 0.96 & 0.96 & 0.95 & 0.95 & 0.96 & 0.99 & 0.96 & 0.96 & 0.99 & 0.96 & 0.96 & 0.99 & 0.96\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & 0.99 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.84 & 0.87 & 0.92 & \textbf{0.98}  & 0.87 & 0.93 & 0.84 & 0.87 & 0.92 & 0.95 & 0.87 & 0.93 & 0.84 & 0.87 & 0.92\\
			\texttt{proc} & 0.76 & 0.62 & 0.83 & \textbf{1.00}  & 0.98 & \textbf{0.99}  & 0.74 & 0.53 & 0.82 & \textbf{1.00}  & 0.98 & \textbf{0.99}  & 0.74 & 0.68 & 0.86\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.97 & 0.99 & 0.97 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & 0.99 & 0.99 & 0.97 & 0.99 & 0.97\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.73}  & \textbf{1.00}  & {\color{red} 0.76} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & 0.98 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.44 & \textbf{1.00}  & 0.89 & 0.44 & \textbf{1.00}  & 0.89 & 0.44 & \textbf{1.00}  & 0.89 & 0.44 & \textbf{1.00}  & 0.89 & 0.44 & \textbf{1.00}  & 0.89\\
			\texttt{proc} & 0.44 & \textbf{1.00}  & 0.90 & 0.44 & \textbf{1.00}  & 0.90 & 0.44 & \textbf{1.00}  & 0.90 & 0.44 & \textbf{1.00}  & 0.90 & 0.44 & \textbf{1.00}  & 0.90\\
			\bottomrule
	\end{tabular}}
	
	\caption{BPI Challenge 2015, Sub-Dataset A + RipperK}\label{tab:BPIc15SubARipperK}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & 0.97 & \textbf{1.00}  & 0.97 & 0.96 & \textbf{1.00}  & 0.97 & 0.96 & \textbf{1.00}  & 0.97 & 0.96 & \textbf{1.00}  & 0.97 & 0.96 & \textbf{1.00}  & 0.97\\
			\texttt{mr\_tr} & 0.97 & \textbf{1.00}  & 0.99 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & 0.98 & 0.99 & 0.99 & 0.98 & 0.99 & 0.99 & 0.98 & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.80 & {\color{red} 0.12}  & 0.56 & 0.79 & 0.31 & 0.65 & 0.40 & 0.17 & 0.58 & 0.73 & 0.25 & 0.61 & 0.40 & 0.17 & 0.58\\
			\texttt{proc} & 0.79 & 0.65 & 0.81 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.81 & 0.71 & 0.84 & \textbf{1.00}  & 0.92 & 0.96 & 0.73 & 0.71 & 0.84\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.71}  & {\color{red} 0.95}  & {\color{red} 0.59}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.76}  & {\color{red} 0.74}  & {\color{red} 0.64}  & 0.97 & \textbf{1.00}  & 0.97\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.78}  & {\color{red} 0.45}  & {\color{red} 0.67}  & 0.99 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.93}  & {\color{red} 0.92}  & {\color{red} 0.90}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & \textbf{0.84}  & 0.14 & {\color{red} 0.57}  & 0.44 & \textbf{1.00}  & 0.89 & 0.79 & 0.42 & 0.71 & 0.45 & \textbf{1.00}  & \textbf{0.90} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & 0.97 & \textbf{1.00}  & 0.97 & 0.97 & \textbf{1.00}  & 0.97 & 0.96 & \textbf{1.00}  & 0.97 & 0.97 & \textbf{1.00}  & 0.97 & 0.96 & \textbf{1.00}  & 0.97\\
			\texttt{mr\_tr} & \textbf{1.00}  & 0.51 & 0.76 & 0.99 & 0.95 & 0.97 & \textbf{1.00}  & 0.55 & 0.78 & 0.99 & 0.93 & 0.96 & \textbf{1.00}  & 0.57 & 0.79\\
			\texttt{mra\_tra} & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & \textbf{0.84}  & 0.62 & 0.80 & 0.69 & 0.42 & 0.69 & 0.69 & 0.42 & 0.69 & {\color{red} 0.35}  & 0.42 & 0.67 & 0.69 & 0.42 & 0.69\\
			\texttt{proc} & 0.80 & 0.68 & 0.83 & 0.50 & 0.50 & 0.74 & 0.77 & 0.68 & 0.83 & 0.98 & 0.92 & 0.96 & 0.41 & 0.71 & 0.62\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.97 & 0.99 & 0.97 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.97 & 0.99 & 0.97 & 0.99 & 0.99 & 0.99\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.45 & \textbf{1.00}  & \textbf{0.90}  & 0.47 & \textbf{1.00}  & \textbf{0.90}  & 0.44 & \textbf{1.00}  & 0.89 & 0.45 & \textbf{1.00}  & \textbf{0.90}  & 0.44 & \textbf{1.00}  & 0.89\\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
\end{table}

\begin{table}
	\caption{BPI Challenge 2015, Sub-Dataset B + Decision Tree}\label{tab:BPIc15SubDecision Tree}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & 0.98 & 0.98 & 0.97 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.99 & 0.99 & 0.99 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.98 & 0.99 & 0.99 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.98 & 0.99 & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.54 & 0.40 & {\color{red} 0.68}  & 0.57 & 0.50 & 0.72 & 0.59 & {\color{red} 0.35}  & 0.76 & 0.59 & 0.40 & 0.74 & 0.58 & 0.40 & {\color{red} 0.68} \\
			\texttt{proc} & 0.49 & 0.37 & {\color{red} 0.67}  & \textbf{1.00}  & 0.78 & 0.95 & 0.49 & 0.37 & {\color{red} 0.67}  & 0.95 & 0.78 & 0.93 & 0.49 & 0.37 & {\color{red} 0.67} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.98 & 0.99 & {\color{red} 0.94}  & {\color{red} 0.91}  & {\color{red} 0.88}  & \textbf{1.00}  & 0.99 & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.92}  & {\color{red} 0.92}  & {\color{red} 0.88}  & 0.99 & \textbf{1.00}  & 0.99\\
			\texttt{mr\_tr} & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.93}  & {\color{red} 0.91}  & {\color{red} 0.92}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.92}  & {\color{red} 0.92}  & {\color{red} 0.82}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & {\color{red} 0.47}  & \textbf{1.00}  & \textbf{0.93}  & {\color{red} 0.47}  & \textbf{1.00}  & \textbf{0.93}  & 0.87 & 0.66 & 0.82 & {\color{red} 0.47}  & \textbf{1.00}  & \textbf{0.93} \\
			\texttt{proc} & 0.73 & \textbf{1.00}  & 0.96 & 0.73 & \textbf{1.00}  & 0.96 & {\color{red} 0.43}  & 0.28 & 0.72 & 0.73 & \textbf{1.00}  & 0.96\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & 0.98 & 0.98 & 0.97 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.99 & 0.99 & 0.99 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & 0.99 & 0.99 & 0.98 & 0.99 & 0.99 & 0.98 & \textbf{1.00}  & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & \textbf{1.00}  & 0.70 & 0.86 & 0.87 & 0.66 & 0.82 & 0.93 & 0.70 & 0.85 & \textbf{1.00}  & 0.70 & 0.86 & 0.93 & 0.70 & 0.85\\
			\texttt{proc} & 0.57 & {\color{red} 0.23}  & 0.72 & \textbf{1.00}  & 0.78 & \textbf{0.97}  & 0.70 & 0.32 & 0.77 & 0.95 & 0.78 & 0.91 & 0.70 & 0.32 & 0.77\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & 0.96\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & {\color{red} 0.47}  & \textbf{1.00}  & \textbf{0.93}  & {\color{red} 0.47}  & \textbf{1.00}  & \textbf{0.93}  & {\color{red} 0.47}  & \textbf{1.00}  & \textbf{0.93}  & {\color{red} 0.47}  & \textbf{1.00}  & \textbf{0.93}  & {\color{red} 0.47}  & \textbf{1.00}  & \textbf{0.93} \\
			\texttt{proc} & 0.73 & \textbf{1.00}  & 0.96 & 0.45 & \textbf{1.00}  & 0.91 & 0.45 & \textbf{1.00}  & 0.91 & 0.45 & \textbf{1.00}  & 0.91 & 0.73 & \textbf{1.00}  & 0.96\\
			\bottomrule
	\end{tabular}}
	
	\caption{BPI Challenge 2015, Sub-Dataset B + RipperK}\label{tab:BPIc15SubRipperK}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & 0.98 & \textbf{1.00}  & 0.98 & 0.98 & \textbf{1.00}  & 0.98 & 0.98 & \textbf{1.00}  & 0.98 & 0.98 & 0.96 & 0.98 & 0.98 & \textbf{1.00}  & 0.98\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & 0.99 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.45 & 0.45 & 0.69 & {\color{red} 0.41}  & {\color{red} 0.37}  & {\color{red} 0.66}  & 0.54 & 0.45 & 0.70 & 0.73 & 0.45 & 0.71 & 0.50 & 0.44 & 0.69\\
			\texttt{proc} & 0.77 & 0.37 & 0.68 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.76 & {\color{red} 0.32}  & 0.66 & 0.90 & 0.87 & 0.93 & 0.76 & {\color{red} 0.32}  & 0.66\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.97}  & {\color{red} 0.90}  & {\color{red} 0.92}  & \textbf{1.00}  & 0.98 & 0.99\\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.88}  & {\color{red} 0.87}  & {\color{red} 0.82}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.93}  & {\color{red} 0.92}  & {\color{red} 0.95}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.93}  & {\color{red} 0.95}  & {\color{red} 0.88}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.46 & 0.56 & 0.74 & 0.47 & \textbf{1.00}  & \textbf{0.93}  & 0.87 & 0.61 & 0.80 & 0.47 & \textbf{1.00}  & \textbf{0.93} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.69 & 0.50 & 0.73 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & 0.98 & \textbf{1.00}  & 0.98 & 0.98 & \textbf{1.00}  & 0.98 & 0.98 & \textbf{1.00}  & 0.98 & 0.98 & \textbf{1.00}  & 0.98 & 0.98 & \textbf{1.00}  & 0.98\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.96 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.95 & 0.61 & 0.80 & 0.87 & 0.66 & 0.83 & 0.86 & 0.66 & 0.83 & 0.81 & 0.70 & 0.85 & \textbf{1.00}  & 0.70 & 0.86\\
			\texttt{proc} & 0.56 & {\color{red} 0.32}  & {\color{red} 0.65}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.92 & {\color{red} 0.32}  & 0.66 & 0.90 & 0.87 & 0.93 & 0.83 & 0.46 & 0.72\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.97 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.97 & 0.99\\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & 0.99 & 0.99 & \textbf{1.00}  & 0.99 & 0.99 & \textbf{1.00}  & 0.98 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.47 & \textbf{1.00}  & \textbf{0.93}  & 0.47 & \textbf{1.00}  & \textbf{0.93}  & 0.47 & \textbf{1.00}  & \textbf{0.93}  & 0.47 & \textbf{1.00}  & \textbf{0.93}  & 0.47 & \textbf{1.00}  & \textbf{0.93} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
\end{table}

\begin{table}
	\caption{BPI Challenge 2015, Sub-Dataset C + Decision Tree}\label{tab:BPIc15SubCDecision Tree}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.54 & 0.29 & 0.69 & 0.42 & 0.38 & {\color{red} 0.60}  & 0.59 & {\color{red} 0.25}  & 0.67 & 0.41 & 0.32 & {\color{red} 0.60}  & {\color{red} 0.40}  & 0.35 & 0.63\\
			\texttt{proc} & 0.73 & 0.76 & 0.95 & 0.97 & 0.89 & 0.95 & 0.71 & 0.73 & 0.93 & \textbf{1.00}  & 0.98 & \textbf{0.99}  & 0.74 & 0.64 & 0.84\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.85}  & {\color{red} 0.78}  & {\color{red} 0.75}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.82}  & {\color{red} 0.78}  & {\color{red} 0.76}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & {\color{red} 0.76}  & \textbf{1.00}  & {\color{red} 0.76}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.78 & {\color{red} 0.79}  & 0.79 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.86}  & \textbf{1.00}  & {\color{red} 0.76}  & 0.88 & {\color{red} 0.90}  & 0.79 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.45 & \textbf{1.00}  & \textbf{0.93}  & 0.45 & \textbf{1.00}  & \textbf{0.93}  & \textbf{0.93}  & 0.82 & 0.90 & 0.45 & \textbf{1.00}  & \textbf{0.93} \\
			\texttt{proc} & {\color{red} 0.45}  & \textbf{1.00}  & 0.92 & {\color{red} 0.45}  & \textbf{1.00}  & 0.92 & 0.54 & {\color{red} 0.34}  & {\color{red} 0.80}  & {\color{red} 0.45}  & \textbf{1.00}  & 0.92\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & 0.99 & 0.97 & 0.98 & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.97 & 0.99 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.97 & 0.99\\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & 0.99 & 0.99 & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.76 & 0.76 & 0.88 & 0.78 & 0.76 & 0.88 & 0.78 & 0.79 & 0.89 & 0.75 & 0.76 & 0.86 & 0.82 & 0.82 & 0.91\\
			\texttt{proc} & 0.76 & 0.76 & 0.95 & 0.95 & 0.89 & 0.95 & 0.76 & 0.76 & 0.95 & \textbf{1.00}  & 0.98 & \textbf{0.99}  & 0.75 & 0.73 & 0.94\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.98 & \textbf{1.00}  & 0.99 & 0.97 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.98 & \textbf{1.00}  & 0.99 & 0.98 & \textbf{1.00}  & 0.99\\
			\texttt{mra\_tra} & {\color{red} 0.86}  & \textbf{1.00}  & {\color{red} 0.76}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.45 & \textbf{1.00}  & \textbf{0.93}  & 0.45 & \textbf{1.00}  & \textbf{0.93}  & 0.45 & \textbf{1.00}  & \textbf{0.93}  & 0.45 & \textbf{1.00}  & \textbf{0.93}  & 0.45 & \textbf{1.00}  & \textbf{0.93} \\
			\texttt{proc} & {\color{red} 0.45}  & \textbf{1.00}  & 0.92 & {\color{red} 0.45}  & \textbf{1.00}  & 0.92 & {\color{red} 0.45}  & \textbf{1.00}  & 0.92 & {\color{red} 0.45}  & \textbf{1.00}  & 0.92 & {\color{red} 0.45}  & \textbf{1.00}  & 0.92\\
			\bottomrule
	\end{tabular}}
	\caption{BPI Challenge 2015, Sub-Dataset C + RipperK}\label{tab:BPIc15SubCRipperK}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & 0.98 & \textbf{1.00}  & \textbf{1.00}  & 0.94 & 0.98 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.43 & {\color{red} 0.10}  & {\color{red} 0.54}  & 0.52 & 0.35 & 0.65 & 0.46 & 0.16 & 0.56 & 0.28 & {\color{red} 0.10}  & {\color{red} 0.54}  & 0.46 & {\color{red} 0.10}  & {\color{red} 0.54} \\
			\texttt{proc} & 0.72 & 0.73 & 0.85 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.87 & 0.67 & 0.83 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.77 & 0.73 & 0.85\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.80}  & {\color{red} 0.81}  & {\color{red} 0.73}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.85}  & {\color{red} 0.86}  & {\color{red} 0.80}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.98 & \textbf{1.00}  & 0.99 & 0.98 & \textbf{1.00}  & 0.99 & {\color{red} 0.79}  & {\color{red} 0.86}  & {\color{red} 0.81}  & 0.98 & \textbf{1.00}  & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.84}  & {\color{red} 0.99}  & {\color{red} 0.75}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00} \\
			\texttt{payload} & 0.59 & 0.22 & 0.60 & 0.45 & \textbf{1.00}  & 0.93 & \textbf{0.93}  & 0.85 & 0.92 & 0.45 & \textbf{1.00}  & 0.93\\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.67}  & {\color{red} 0.31}  & {\color{red} 0.64}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & \textbf{0.93}  & 0.85 & 0.92 & 0.87 & 0.85 & 0.92 & 0.90 & 0.85 & 0.92 & 0.85 & 0.88 & \textbf{0.94}  & \textbf{0.93}  & 0.85 & 0.92\\
			\texttt{proc} & 0.80 & 0.81 & 0.89 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.78 & 0.39 & 0.69 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.70 & 0.81 & 0.89\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.98 & \textbf{1.00}  & 0.99 & 0.98 & \textbf{1.00}  & 0.99 & 0.98 & \textbf{1.00}  & 0.99 & 0.98 & \textbf{1.00}  & 0.99 & 0.98 & \textbf{1.00}  & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.99}  & \textbf{1.00} \\
			\texttt{payload} & 0.45 & \textbf{1.00}  & 0.93 & 0.45 & \textbf{1.00}  & 0.93 & 0.45 & \textbf{1.00}  & 0.93 & 0.45 & \textbf{1.00}  & 0.93 & 0.45 & \textbf{1.00}  & 0.93\\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
\end{table}

%

\begin{table}
	\caption{BPI Challenge 2015, Sub-Dataset D + Decision Tree}\label{tab:BPIc15SubDDecision Tree}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.98 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & 0.98 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.34 & 0.07 & {\color{red} 0.67}  & 0.85 & 0.37 & 0.68 & {\color{red} 0.33}  & 0.10 & 0.70 & 0.65 & 0.54 & 0.75 & 0.58 & 0.10 & 0.70\\
			\texttt{proc} & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.46}  & 0.96 & 0.92 & 0.99 & 0.08 & 0.05 & {\color{red} 0.46}  & \textbf{1.00}  & 0.80 & \textbf{1.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.46} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.82}  & {\color{red} 0.77}  & {\color{red} 0.70}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & {\color{red} 0.83}  & {\color{red} 0.89}  & {\color{red} 0.75}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.77}  & {\color{red} 0.93}  & {\color{red} 0.86}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.96 & 0.98 & {\color{red} 0.30}  & {\color{red} 0.22}  & {\color{red} 0.60}  & \textbf{1.00}  & 0.96 & 0.98\\
			\texttt{payload} & 0.47 & \textbf{1.00}  & 0.91 & 0.47 & \textbf{1.00}  & 0.91 & \textbf{1.00}  & 0.97 & \textbf{0.99}  & 0.47 & \textbf{1.00}  & 0.91\\
			\texttt{proc} & 0.43 & \textbf{1.00}  & 0.92 & 0.43 & \textbf{1.00}  & 0.92 & 0.27 & 0.09 & 0.58 & 0.43 & \textbf{1.00}  & 0.92\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.96 & \textbf{1.00}  & 0.98 & 0.98 & \textbf{1.00}  & 0.99 & 0.96 & \textbf{1.00}  & 0.98 & 0.96 & \textbf{1.00}  & 0.98 & \textbf{1.00}  & 0.99 & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & \textbf{1.00}  & 0.97 & \textbf{0.99}  & 0.97 & 0.97 & \textbf{0.99}  & \textbf{1.00}  & 0.97 & \textbf{0.99}  & \textbf{1.00}  & 0.97 & \textbf{0.99}  & \textbf{1.00}  & 0.97 & \textbf{0.99} \\
			\texttt{proc} & 0.17 & 0.09 & 0.62 & 0.96 & 0.88 & 0.97 & 0.15 & 0.09 & 0.62 & 0.96 & 0.80 & 0.90 & 0.16 & 0.09 & 0.62\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.47 & \textbf{1.00}  & 0.91 & 0.47 & \textbf{1.00}  & 0.91 & 0.47 & \textbf{1.00}  & 0.91 & 0.47 & \textbf{1.00}  & 0.91 & 0.47 & \textbf{1.00}  & 0.91\\
			\texttt{proc} & 0.43 & \textbf{1.00}  & 0.92 & 0.43 & \textbf{1.00}  & 0.92 & 0.43 & \textbf{1.00}  & 0.92 & 0.43 & \textbf{1.00}  & 0.92 & 0.43 & \textbf{1.00}  & 0.92\\
			\bottomrule
	\end{tabular}}
	
	\caption{BPI Challenge 2015, Sub-Dataset D + RipperK}\label{tab:BPIc15SubDRipperK}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.98 & 0.98 & 0.97 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & 0.96 & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & {\color{red} 0.39}  & 0.14 & 0.56 & 0.63 & 0.54 & 0.75 & 0.50 & 0.07 & {\color{red} 0.54}  & 0.64 & 0.57 & 0.76 & 0.50 & 0.07 & {\color{red} 0.54} \\
			\texttt{proc} & 0.17 & 0.13 & 0.54 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.00}  & 0.13 & 0.54 & 0.93 & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.00}  & 0.13 & 0.54\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.80}  & {\color{red} 0.83}  & {\color{red} 0.69}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & {\color{red} 0.84}  & {\color{red} 0.82}  & {\color{red} 0.76}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.76}  & {\color{red} 0.93}  & {\color{red} 0.83}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & 0.96 & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.50}  & {\color{red} 0.40}  & {\color{red} 0.68}  & 0.96 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.76 & 0.44 & 0.71 & 0.47 & \textbf{1.00}  & 0.91 & \textbf{1.00}  & 0.97 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.10 & {\color{red} 0.09}  & {\color{red} 0.52}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & 0.99 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.94 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & 0.96 & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.96 & 0.98 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.96 & 0.96 & 0.98\\
			\texttt{payload} & \textbf{1.00}  & 0.97 & 0.99 & \textbf{1.00}  & 0.97 & 0.99 & \textbf{1.00}  & 0.97 & 0.99 & \textbf{1.00}  & 0.97 & 0.99 & \textbf{1.00}  & 0.97 & 0.99\\
			\texttt{proc} & {\color{red} 0.00}  & 0.17 & 0.57 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.00}  & 0.25 & 0.61 & 0.97 & 0.84 & 0.92 & 0.50 & 0.25 & 0.61\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & 0.96 & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.47 & \textbf{1.00}  & 0.91 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.47 & \textbf{1.00}  & 0.91 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
\end{table}




\begin{table}
	\caption{BPI Challenge 2015, Sub-Dataset E + Decision Tree}\label{tab:BPIc15SubEDecision Tree}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & 0.95 & 0.98 & 0.94 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.98 & 0.99\\
			\texttt{mr\_tr} & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & 0.98 & 0.98 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.98 & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.25 & 0.17 & 0.70 & 0.58 & 0.80 & 0.85 & {\color{red} 0.17}  & {\color{red} 0.05}  & {\color{red} 0.67}  & 0.65 & 0.76 & 0.82 & {\color{red} 0.17}  & {\color{red} 0.05}  & {\color{red} 0.67} \\
			\texttt{proc} & 0.58 & 0.37 & 0.75 & 0.96 & 0.91 & 0.96 & 0.79 & 0.37 & 0.76 & 0.96 & 0.96 & \textbf{0.98}  & 0.53 & 0.41 & 0.78\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%	\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.86}  & {\color{red} 0.90}  & {\color{red} 0.80}  & 0.97 & \textbf{1.00}  & 0.97\\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.80}  & {\color{red} 0.81}  & {\color{red} 0.72}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.86}  & {\color{red} 0.80}  & {\color{red} 0.85}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.95}  & {\color{red} 0.95}  & {\color{red} 0.91}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.43 & \textbf{1.00}  & 0.93 & 0.43 & \textbf{1.00}  & 0.93 & \textbf{0.93}  & 0.88 & \textbf{0.94}  & 0.43 & \textbf{1.00}  & 0.93\\
			\texttt{proc} & 0.73 & \textbf{1.00}  & 0.97 & {\color{red} 0.46}  & \textbf{1.00}  & 0.94 & 0.50 & {\color{red} 0.19}  & {\color{red} 0.63}  & 0.73 & \textbf{1.00}  & 0.97\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00} \\
			\texttt{decl} & 0.95 & 0.98 & 0.96 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & 0.99 & \textbf{1.00}  & 0.99 & 0.98 & 0.98 & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.81 & 0.88 & 0.93 & 0.81 & 0.88 & 0.93 & 0.81 & 0.88 & 0.93 & 0.76 & 0.88 & 0.93 & 0.81 & 0.88 & 0.93\\
			\texttt{proc} & 0.49 & 0.50 & 0.78 & 0.96 & 0.91 & 0.96 & 0.79 & 0.37 & 0.79 & \textbf{1.00}  & 0.96 & \textbf{0.98}  & 0.79 & 0.37 & 0.79\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.97 & \textbf{1.00}  & 0.97 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.97 & \textbf{1.00}  & 0.97 & 0.97 & \textbf{1.00}  & 0.97\\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.96 & \textbf{1.00}  & 0.96 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.43 & \textbf{1.00}  & 0.93 & 0.43 & \textbf{1.00}  & 0.93 & 0.43 & \textbf{1.00}  & 0.93 & 0.43 & \textbf{1.00}  & 0.93 & 0.43 & \textbf{1.00}  & 0.93\\
			\texttt{proc} & {\color{red} 0.46}  & \textbf{1.00}  & 0.94 & {\color{red} 0.46}  & \textbf{1.00}  & 0.94 & 0.73 & \textbf{1.00}  & 0.97 & 0.73 & \textbf{1.00}  & 0.97 & {\color{red} 0.46}  & \textbf{1.00}  & 0.94\\
			\bottomrule
	\end{tabular}}
	
	\caption{BPI Challenge 2015, Sub-Dataset E + RipperK}\label{tab:BPIc15SubERipperK}
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{IA} & \multicolumn{3}{c}{MR} & \multicolumn{3}{c}{TR} & \multicolumn{3}{c}{MRA} & \multicolumn{3}{c}{TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & 0.95 & \textbf{1.00}  & 0.96 & 0.95 & \textbf{1.00}  & 0.96 & 0.95 & \textbf{1.00}  & 0.96 & 0.95 & \textbf{1.00}  & 0.96 & 0.95 & \textbf{1.00}  & 0.96\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.97 & \textbf{1.00}  & 0.99 & 0.97 & \textbf{1.00}  & 0.99 & 0.97 & \textbf{1.00}  & 0.99 & 0.97 & \textbf{1.00}  & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & 0.23 & 0.21 & 0.58 & 0.67 & 0.76 & 0.86 & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00}  & 0.61 & 0.80 & 0.88 & {\color{red} 0.00}  & {\color{red} 0.00}  & {\color{red} 0.00} \\
			\texttt{proc} & 0.90 & 0.41 & 0.71 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.79 & 0.41 & 0.70 & 0.96 & \textbf{1.00}  & \textbf{1.00}  & 0.79 & 0.41 & 0.70\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Declare} & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{Data} & \multicolumn{3}{c}{DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.85}  & {\color{red} 0.94}  & {\color{red} 0.80}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.81}  & {\color{red} 0.82}  & {\color{red} 0.78}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mr\_tr} & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.88}  & {\color{red} 0.80}  & {\color{red} 0.86}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & 0.99 & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.98 & {\color{red} 0.95}  & {\color{red} 0.98}  & {\color{red} 0.91}  & 0.99 & \textbf{1.00}  & 0.98\\
			\texttt{payload} & 0.76 & 0.80 & 0.88 & 0.44 & \textbf{1.00}  & 0.93 & \textbf{0.93}  & 0.88 & \textbf{0.94}  & 0.43 & \textbf{1.00}  & 0.93\\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & {\color{red} 0.38}  & 0.14 & 0.56 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+IA} & \multicolumn{3}{c}{Data+MR} & \multicolumn{3}{c}{Data+TR} & \multicolumn{3}{c}{Data+MRA} & \multicolumn{3}{c}{Data+TRA} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & 0.95 & \textbf{1.00}  & 0.96 & 0.95 & \textbf{1.00}  & 0.96 & 0.95 & \textbf{1.00}  & 0.96 & 0.95 & \textbf{1.00}  & 0.96 & 0.95 & \textbf{1.00}  & 0.96\\
			\texttt{mr\_tr} & 0.95 & \textbf{1.00}  & \textbf{1.00}  & 0.97 & \textbf{1.00}  & 0.99 & 0.99 & \textbf{1.00}  & 0.99 & 0.99 & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & 0.99\\
			\texttt{mra\_tra} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.99 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{payload} & \textbf{0.93}  & 0.88 & \textbf{0.94}  & \textbf{0.93}  & 0.88 & \textbf{0.94}  & \textbf{0.93}  & 0.88 & \textbf{0.94}  & \textbf{0.93}  & 0.88 & \textbf{0.94}  & \textbf{0.93}  & 0.88 & \textbf{0.94} \\
			\texttt{proc} & 0.68 & 0.41 & 0.70 & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.90 & 0.28 & 0.64 & \textbf{1.00}  & 0.91 & 0.96 & 0.90 & 0.28 & 0.64\\
			\bottomrule
	\end{tabular}}
	
	
	{\tiny\begin{tabular}{l|lll|lll|lll|lll|lll}
			\toprule
			\multirow{2}{*}{Labelling} & \multicolumn{3}{c}{Data+Declare} & \multicolumn{3}{c}{Data+DeclD} & \multicolumn{3}{c}{Data+H} & \multicolumn{3}{c}{H+DeclD} & \multicolumn{3}{c}{H+Data+DeclD} \\
			{}  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC  & Prec & Rec & AUC \\
			\midrule
			%\texttt{decl2} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{decl} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & 0.97 & \textbf{1.00}  & 0.97\\
			\texttt{mr\_tr} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\texttt{mra\_tra} & 0.99 & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.98 & 0.99 & \textbf{1.00}  & 0.98\\
			\texttt{payload} & 0.64 & 0.96 & \textbf{0.94}  & \textbf{0.93}  & 0.76 & 0.88 & 0.64 & 0.96 & \textbf{0.94}  & \textbf{0.93}  & 0.76 & 0.88 & \textbf{0.93}  & 0.76 & 0.88\\
			\texttt{proc} & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00}  & \textbf{1.00} \\
			\bottomrule
	\end{tabular}}
\end{table}


==> threats.tex <==
% !TEX root = paper.tex
\section{Threats to validity}
\label{sec:threats}

One of the threats to the validity of this study relates to the potential selection bias in the literature review. To minimize this, we described our systematic literature review procedure on a level of detail that is sufficient to replicate the search. However, in time the search and ranking algorithms of the used academic database (Google Scholar) might be updated and return different results. Another potential source of bias is the subjectivity when applying inclusion and exclusion criteria, as well as when determining the primary and subsumed studies. In order to alleviate this issue, all the included papers were collected in a publicly available spreadsheet, together with decisions and reasons about excluding them from the study. Moreover, each paper was independently assessed against the inclusion and exclusion criteria by two authors, and inconsistencies were resolved with the mediation of a third author.  

Another threat to validity is related to the comprehensiveness of the conducted experiments. In particular, only one clustering method was tested, a single state abstraction was used when building the transition systems for state-based bucketing, and four classification algorithms were applied. It is possible that there exists, for example, a combination of an untested clustering technique and a classifier that outperforms the settings used in this study. Also, although the hyperparameters were optimized using a state-of-the-art hyperparameter optimization technique, it is possible that using more iterations for optimization or a different optimization algorithm, other parameter settings would be found that outperform the settings used in the current evaluation. 
%In particular, only one representative setting of each technique was used, with minimal hyperparameter optimization. Namely, only one clustering method was tested, a single state abstraction was used when building the transition systems for state-based bucketing, and one classification algorithm was used over all methods. It is possible that there exists, for example, a combination of an untested clustering technique and a classifier that outperforms the settings used in this study. 
Furthermore, the generalizability of the findings is to some extent limited by the fact that the experiments were performed on a limited number of prediction tasks (24), constructed from nine event logs. Although these are all real-life event logs from different application fields that exhibit different characteristics, it may be possible that the results would be different using other datasets or different log preprocessing techniques for the same datasets. In order to mitigate these threats, we built an open-source software framework which allows the full replication of the experiments, and made this tool publicly available. Moreover, additional datasets, as well as new sequence classification and encoding methods can be plugged in. So the framework can be used for future experiments. Also, the preprocessed datasets constructed from the three publicly available event logs are included together with the tool implementation in order to enhance the reproducibility of the experiments.

%A potential threat to validity is that when measuring prediction accuracy of multi-bucket methods, the prediction scores coming from different classifiers (buckets) are mixed together ``as is'' and ordered to measure AUC. However, it may be possible that different classifiers return prediction scores that are on different scales, making it necessary to \emph{calibrate} the predictions. However, as the aim of this study is to compare existing methods as they were proposed (without any calibration), this questions is rather a direction for future work.  


==> tikzlibraryDECLARE.code.tex <==
%
% This is the DECLARE TikZ library by Claudio Di Ciccio is licensed under a Creative Commons Attribution-ShareAlike 4.0 International License.
% This work is licensed under the Creative Commons Attribution-ShareAlike 4.0 International License. To view a copy of this license, visit http://creativecommons.org/licenses/by-sa/4.0/.
%
% Author: Claudio Di Ciccio
% Website: www.diciccio.net
% Date: 2017/02/08
%
\usetikzlibrary{arrows.meta,decorations.markings}
\def\DTZU {2ex}
\tikzset{
 DECLARE.task/.style={
  rounded corners=1,
  minimum width=3em,
  minimum height=1ex,
  draw
 },
 DECLARE.existcon/.style={
  label={[style=draw,yshift=-1\pgflinewidth]above:{\tiny \textit{#1}}}
 },
 DECLARE.neg/.style={
  semithick,
  postaction={decorate,decoration={markings,
   mark=at position .5 with {\arrow[xshift=0.15*\DTZU]{Bar[width=1.5*\DTZU]}},
   mark=at position .5 with {\arrow[xshift=-0.15*\DTZU]{Bar[width=1.5*\DTZU]}}
  }}
 },
 DECLARE.resex/.style={
  semithick,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-,
  shorten <=-0.5*\DTZU
 },
 DECLARE.resp/.style={
  semithick,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU
 },
 DECLARE.alt.resp/.style={
  semithick,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  double distance=0.25*\DTZU
 },
 DECLARE.chn.resp/.style={
  semithick,
  preaction={draw, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}
 },
 DECLARE.prec/.style={
  semithick,
  {-{Triangle[length=1*\DTZU,width=1*\DTZU]Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >=-0.5*\DTZU
 },
 DECLARE.alt.prec/.style={
  semithick,
  postaction={draw, shorten >= 0.5*\DTZU, double distance=0.25*\DTZU, {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.chn.prec/.style={
  semithick,
  preaction={draw, shorten >= 0.5*\DTZU, double distance=0.25*\DTZU, {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.succ/.style={
  semithick,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]Circle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  shorten >=-0.5*\DTZU
 },
 DECLARE.coex/.style={
  semithick,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Circle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  shorten >=-0.5*\DTZU
 },
 DECLARE.alt.succ/.style={
  semithick,
  postaction={draw, shorten >= 0.5*\DTZU, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.chn.succ/.style={
  semithick,
  preaction={draw, shorten >= 0.5*\DTZU, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 }
}
